An efficient computational framework for naval shape design and optimization problems by means of data-driven reduced order modeling techniques

This contribution describes the implementation of a data--driven shape optimization pipeline in a naval architecture application. We adopt reduced order models (ROMs) in order to improve the efficiency of the overall optimization, keeping a modular and equation-free nature to target the industrial demand. We applied the above mentioned pipeline to a realistic cruise ship in order to reduce the total drag. We begin by defining the design space, generated by deforming an initial shape in a parametric way using free form deformation (FFD). The evaluation of the performance of each new hull is determined by simulating the flux via finite volume discretization of a two-phase (water and air) fluid. Since the fluid dynamics model can result very expensive -- especially dealing with complex industrial geometries -- we propose also a dynamic mode decomposition (DMD) enhancement to reduce the computational cost of a single numerical simulation. The real--time computation is finally achieved by means of proper orthogonal decomposition with Gaussian process regression (POD-GPR) technique. Thanks to the quick approximation, a genetic optimization algorithm becomes feasible to converge towards the optimal shape.

==> sections/abstract.tex <==

\begin{abstract}
This contribution describes the implementation of a data--driven shape
	optimization pipeline in a naval architecture application. We adopt
	reduced order models (ROMs) in order to improve the efficiency of the
	overall optimization, keeping a modular and equation-free nature to
	target the industrial demand.  We applied the above mentioned pipeline
	to a realistic cruise ship in order to reduce the total drag. We begin
	by defining the design space, generated by deforming an initial shape
	in a parametric way using free form deformation (FFD). The evaluation
	of the performance of each new hull is determined by simulating the
	flux via finite volume discretization of a two-phase (water and air)
	fluid. Since the fluid dynamics model can result very expensive ---
	especially dealing with complex industrial geometries --- we propose also
	a dynamic mode decomposition (DMD) enhancement to reduce the
	computational cost of a single numerical simulation. The real--time
	computation is finally achieved by means of proper orthogonal
	decomposition with Gaussian process regression (POD-GPR) technique.
	Thanks to the quick approximation, a genetic optimization algorithm
	becomes feasible to converge towards the optimal shape.
\keywords{
	Finite volume method \and 
	Computational fluid dynamics \and
	Data-driven reduced order modeling \and 
	Free form deformation \and
	Shape optimization
}
\end{abstract}


==> sections/results.tex <==

\section{Numerical results: a cruise ship shape optimization}
\label{sec:results}

In this section, we will present the results obtained by applying the described
computational pipeline to optimize the shape of a cruise ship.
We maintain the same structure
of the previous section, discussing the intermediate results for any mentioned
technique.
\begin{figure}[h]
\centering
\includegraphics[width=.5\textwidth]{figures/boat.png}
\caption{The undeformed hull.}
\label{boat}
\end{figure}

\paragraph{Free-form deformation}
We set the domain $D$, aka the space enclosed by the lattice of FFD control points, in order to deform only the immersed part of the hull, in the proximity of the bow.
The lattice is illustrated in \autoref{grid2}, and we can see that it is
positioned, in $x$ direction, on sections $10, 12, 14, 16, 18, 20$ and
22\footnote{In naval architecture a boat is divided, no matter the size, in $20$
chunks, generated by $21$ equally spaced cuts obtained with planes perpendicular
to the $x$-axis}. For $z$ direction, the points are displaced around the
waterline, while along $y$ axis the points are positioned for the entire width
of the ship. In total, $539$ FFD points are used.
\begin{figure}[h]
\centering
\includegraphics[width=.5\textwidth]{figures/grid2.png}
\includegraphics[width=.5\textwidth]{figures/grid1.png}
\caption{$x$- and $y$-normal view of the set $D$ (in blue) and the lattice of points $P^0_{l,m,n}$ (in red) over the undeformed hull.}
\label{grid2}
\end{figure}

Concerning the motion of such points only part of the points in the lattice are
displaced: we use $6$ parameters to control the movements along $x$ (the first
three parameters) and along $y$. An example of this motion is sketched in
\autoref{fig:ffd_ex}, where red arrows refers to control points movements. The layers corresponding to sections $10, 12,
20$ and $22$ remain fixed, together with the two upper and lower layers, the
two far left and the two far-right layers and, finally, the layer over the
longitudinal symmetry plane. Except for this last one, that is kept fixed to
maintain symmetry, the other layers are kept fixed in order to achieve the
continuity and smoothness of the shapes, required especially in the $x$
direction where the deformation must link in a smooth way to the rest of the
boat.

\begin{figure}[h]
\centering
\includegraphics[width=.5\textwidth]{figures/53.png}
\caption{Example of shape morphing with $\mupar~=~[0.08, 0.08, -0.06, 0.08, -0.08, 0.08]$}
\label{fig:ffd_ex}
\end{figure}

The parameter range have been chosen in order to avoid a high decrease of the
hull volume and, at the same time, explores a large variety of new shapes. In
details, we have a tolerance of the $1\permil$ for the volume constraint. With
a trial and error approach we define the parameter ranges, obtaining a
parameter space  that is $P = [-0.08, 0.08]^6$ (the dimension of such space is
the number of parameters, $6$ in this test).
We underline that the parameters refer to the motion normalized for the $D$
length along the corresponding direction.

We create a set of $100$ samples taking with uniform distribution on the
parametric space. These are the input parameters of the high-fidelity database
required for ROM.

\paragraph{Finite volume discretization}
We simulate the flow pasting around the ship using the FV method, computing for
each deformed object the distribution of the total resistance over the hull.
The simulations are run on model scale ($1:25$).
The computational grid (defined in $[-39,24]\times[-29,0]\times[-24,6]$) is
built from scratch around all the deformed hulls, enforcing the mesh
quality. The computational grid counts $\approx\num{1.5e6}$ cells. To the VOF
model, we need an extra refinement around the waterline in order to avoid a
diffusive behavior of the fraction variable $\alpha$, which is discontinuous. A
region of the computation grid is reported in \autoref{fig:mesh} for
demonstrative purpose.
\begin{figure}[!t]
\centering
\includegraphics[width=.5\textwidth]{figures/m1.png}
\caption{The refined computational grid}
\label{fig:mesh}
\end{figure}
The numerical schemes adopted are mentioned in \autoref{sec:fom}, and we report
in \autoref{tab:fom} the main physical quantities we fix in our setting. The
Reynolds number is near to $\num{2e7}$.
\begin{table}[b]
\caption{Summary of the numerical variable for VOF-RANS model\label{tab:fom}}
\begin{tabular}{rl}
	inlet velocity $u$ & $\SI{2.26336}{\meter\per\second}$\\
	water density $\rho_W$ & $\SI{1.09e-6}{\meter^2\per\second}$\\
	air density $\rho_A$ & $\SI{1.09e-5}{\meter^2\per\second}$\\
	water kinematic viscosity $\nu_W$ & $\SI{998.8}{\kilogram\per\meter^3}$\\
	air kinematic viscosity $\nu_A$ & $\SI{1}{\kilogram\per\meter^3}$\\
	dissipation rate $\omega$ & $\SI{70.49721}{\second^{-1}}$\\
	turbulent kinetic energy $k$ & $\SI{7.6841e-4}{\meter^2\per\second^2}$\\
\end{tabular}
\end{table}
The integration in time is carried out for $t \in [0, 40]~\si{\second}$, with an initial
step of $\Delta t = \SI{1e-3}{\second}$ and an adjustable time-stepping governed by the
Courant number (we impose it to be lower than $5$). We clarify that, even if
the time stepping is not fixed, we save the equispaced temporal snapshots of
the system in order to feed the DMD algorithm.
In this work, we are interested to the total resistance of the ship: after
computing the pressure, velocity and fraction variable unknowns (from the
VOF-RANS model), we can exploit them in order to calculate the resistance distribution
(both the viscous and the friction terms) over the hull surface.
Regarding the computing time, on a parallel architecture with $40$ processes,
the simulation lasts approximately $8$ hours.

\paragraph{Dynamic mode decomposition}
We applied DMD on the results of the FOM. It is important to specify that we
fit a DMD model for each geometric deformation, as a sort of post-processing on
the output. We train the model using the snapshots $\{\out_i\}_{i=0}^{40}$ for
$i = t_\text{dmd}^0+i\Delta t_\text{dmd}$, with $t_\text{dmd}^0 = \SI{20}{s}, \Delta
t_\text{dmd} = \SI{0.5}{s}$. The first $\SI{20}{s}$ of the simulation are discarded since
they are not particularly meaningful for the boundary conditions propagation.
\begin{figure}[ht]
\centering
\input{plots/eigs.tikz}
\caption{First 5 DMD eigenvalues for a single simulation.}
\label{fig:eigs}
\end{figure}
In this contribution, we analyze the DMD operator from a spectral perspectives.
\autoref{fig:eigs} reports in fact the eigenvalues (computed for a single
simulation) after projecting the output onto a POD space of dimension $5$. The
position of eigenvalues in the complex plane provide information about the
dynamics of all the DMD modes. In particular, the imaginary part is related to
frequency, while the distance between them and the unit circle is related to
the growth-rate. We can neglect the dumped modes (the two eigenvalues inside
the circle) since their contribution is useless for future dynamics and focus
on the remaining ones: two modes present a stable oscillatory trend, that actually
catch the asymptotic oscillations of the FOM, and the last one ($1 + 0i$) is
practically constant. 
We isolate the contribution of only this latter mode, assuming it represents
the regime state to which the FOM converges, using it as final output.  In our
setting, having built the computational grid for all the deformed ships from
scratch, we need as last step to project the resistance distribution over the
initial geometry $\pdomain$, in order to ensure same dimensionality for all the
outputs. In our case we use a closest neighbors interpolation.
Thanks to the application of DMD, we can perform fewer time iterations in the
full-order model: in this case we can reduce the simulated seconds from $60$ to
$40$, approximating the regime state with DMD. This of course implies a
reduction of $\sfrac{1}{3}$ of the overall time required to run all the
simulations.

\paragraph{Proper orthogonal decomposition with Gaussian process regression}
We exploit the collected database in order to build a kind of probabilistic
response surface to predict the resistance of new shapes. We remember the
starting set is composed by $100$ input-output pairs $\{(\mupar_i,
\out_i)\}_{i=1}^{100}$, where $\mupar$ is the geometrical parameters provided
to FFD and $\out$ is the resistance distribution over the deformed hull. Of
the entire set, we use the $80\%$ for train the POD-GPR framework and exploit
the remaining pairs to test our method.
Firstly we applied the POD on the snapshots matrix to reduce the dimension of
the output.
\begin{figure}[t]
\centering
\input{plots/sing_POD.tikz}
\caption{Values of $\frac{\sigma_i}{\sigma_0}$ for the first 40 singular values, ordered from the highest to the lowest value.}
\label{sing_POD}
\end{figure}
In this case the singular values extracted are reported in \autoref{sing_POD}
from an energetic perspective. The decay-rate is not very steep, probably due
to the discontinuous component for the VOF variable $\alpha$, which is directly
involved in the resistance computation.
\begin{figure}[b]
\centering
\input{plots/err2modes.tikz}
\caption{Sensitivity analysis on the accuracy of POD-GPR method varying
the number of POD modes used. The number of snapshots is fixed to
$80$.\label{fig:sens_modes}}
\end{figure}
Despite this, the POD allows to remarkably reduce the dimension of the output,
simplifying the next phase.
We exploit the computed modal coefficient in order to optimize the GP, then query for
the new parametric solutions. 
To measure the accuracy, we propose in \autoref{fig:sens_modes} and
\autoref{fig:sens_snaps} two different sensitivity analysis varying the number
of POD modes used to span the reduced space and the number of snapshots to
train the method, respectively. For sake of completeness, we compare the results
with similar data-driven methodologies that involve, instead the GPR, other
interpolation techniques for modal coefficient approximation, as the linear
interpolation one or the radial basis function (RBF) one. 
We propose here the simplest RBF interpolation, but we make the reader aware
that better results can be achieved tuning the smoothness of RBF, producing a
non-interpolating RBF method.
For more details we refer~\cite{mythesis}.
The error refers to the mean relative error computed on the test dataset (of
dimension $20$), using the resistance distribution coming from DMD as truth
solution. The GPR method is able to reach the minimum error respect to the
other interpolation, resulting in a relative error near to $5\%$ adopting $20$
modes, but reducing its accuracy increasing the number of modes. This trend is
shown also by RBF error, that after an initial decreasing, becomes very large
for many modes.
\begin{figure}[b]
\centering
\input{plots/err2snapshots.tikz}
\caption{Sensitivity analysis on the accuracy of POD-GPR method varying
the number of snapshots. The number of POD modes is fixed to
$20$.\label{fig:sens_snaps}}
\end{figure}
Varying the number of snapshots (\autoref{fig:sens_snaps}), the difference
between RBF and GPR is even more evident. While the RBF reaches an error slightly
less than the $8\%$, the GPR is able to stay beyond the $6\%$ with $80$
snapshots. We note that we get the highest difference between the methods using
few snapshots: the GPR shows higher accuracy even with few samples and a
pretty constant trend for database with greater dimension.
\begin{figure}[h]
\centering
\includegraphics[width=.5\textwidth]{figures/ROMFOMfrontal.png}
\caption{Value of total resistance over the bulbous bow for the FOM (on the left) and for the ROM (on the right).}
\label{ROMFOMfrontal}
\end{figure}
Finally, we
conclude with a graphical visualization of the resistance distribution on (a
limited region\footnote{The bulbous bow is one of the region where the pressure
resistance is higher, and then difficult to predict.} of) the hull in
\autoref{ROMFOMfrontal}, comparing the ROM approximation with the FOM
validation. Even if the difference is notable, the reduced model can express
the main physics behaviour of the original model.
Regarding the computational cost reduction, the reduced model can approximate
the parametric solution only sampling an already defined distribution, and even
on a personal laptop it takes no more than few seconds, whereas the FV solver
takes $8$ hours, resulting in a very huge speedup.

\paragraph{Genetic algorithm}
The goal of the entire pipeline is the minimization of the total resistance
(only in the direction of the flow). To ensure feasibility of the deformed
shape from the engineering viewpoint, we add a penalization on the hulls whose
volume is lower that $999\permil$ of the original hull. In other words, we
penalize the configurations that lead a volume decrease greater than
$\sfrac{1}{1000}$ with respect to the original volume. Our optimization problem
reads:
\begin{equation}
\underset{\mupar}{\text{min}}
\left\{
\begin{aligned}
	&\smallint_{\pdomain} \tau_x \rho - p n_x\quad & \text{if} \smallint_{\pdomain}\rho g h &\geq 0.999 \smallint_{\domain} \rho g h\\
	&\infty & \text{otherwise} &\\
\end{aligned}
\right.
	\label{eq:opt}
\end{equation}
where $\tau_x$ is the $x$ component of the (viscous and turbulent) tangential
stresses, $\rho$ is the density of the fluid (computed according to the VOF
model), $p$ is the pressure, $n_x$ is the $x$ component of the normal to the
surface, $g$ is the gravity acceleration and $h$ is the distance between the
surface and the waterline ($\smallint_\domain \rho g h$ results the volume of
the immersed hull using an hydrostatic approach).
To compute the objective function for a generic parameters, we need to perform
the FFD morphing then project the POD-GPR solutions over the deformed ship, in
order to numerically compute such integral. We clarify that with the reduced
order model returns the distribution of viscous and pressure forces over the
hull, that is $\tau \rho - p$ in $\pdomain$. As already mentioned, these methods
have a negligible computational cost, allowing us to optimize the shape in a
very efficient manner.
Despite its easiness of application, GA requires a good tuning of the
hyper-parameters to result successful. In this work, we applied the one point
crossover~\cite{eshelman1993real} for the mate procedure, while for the
mutation a Gaussian mutation~\cite{hinterding1995gaussian} with $\sigma = 0.1$
has been involved.  We set the mate and mutation
probability to $0.8$ and $0.2$, respectively. Moreover, we use an initial population
dimension $N_0 = 200$, reducing it to $N = 30$ during the evolution. The
stopping criteria in this case is the number of generations, which is set to
$15$. Robustness of this setting is proved in \autoref{fig:opt}, where $15$
different runs have been run and, for each run, the optimal shape is plotted
both in terms of resistance and volume. 
\begin{figure}[b]
\centering
\input{plots/opt1vr.tikz}
	\caption{Optimal shapes produced by $15$ different application of GA,
	in terms of resistance and volume as percentage respect to the original
	ship.}
\label{fig:opt}
\end{figure}
We can note in fact that all the runs have converged to the same fitness,
despite the stochastic component of the method itself, ensuring that the
hyper-parameters are set to fully explore the parameter space (and then globally
converge to the optimal point). The penalization we impose avoids the creation
of unfeasible deformations: the optimum of all the runs show a slight decreased
volume, but within the initial tolerance, while the resistance results decreased by
more than the $4\%$.

We specify that this is the optimum for the reduced model. In order to obtain an
accurate value, the optimal parameter can be plug in the pipeline and the
optimal shape is then validated using the full-order FV method. Additionally, this latter
can be insert in the snapshots database and used to enrich the precision of
the POD-GPR model. In our case, after the validation, the gain in term of
resistance is lower with respect to the ROM approximation, but reaching the $3.3\%$ it
results in a very good outcome in the engineering context.

